Robust Online Selection with Uncertain Offer Acceptance

Online advertising has motivated interest in online selection problems. Displaying ads to the right users benefits both the platform (e.g., via pay-per-click) and the advertisers (by increasing their reach). In practice, not all users click on displayed ads, while the platform's algorithm may miss the users most disposed to do so. This mismatch decreases the platform's revenue and the advertiser's chances to reach the right customers. With this motivation, we propose a secretary problem where a candidate may or may not accept an offer according to a known probability $p$. Because we do not know the top candidate willing to accept an offer, the goal is to maximize a robust objective defined as the minimum over integers $k$ of the probability of choosing one of the top $k$ candidates, given that one of these candidates will accept an offer. Using Markov decision process theory, we derive a linear program for this max-min objective whose solution encodes an optimal policy. The derivation may be of independent interest, as it is generalizable and can be used to obtain linear programs for many online selection models. We further relax this linear program into an infinite counterpart, which we use to provide bounds for the objective and closed-form policies. For $p \geq p^* \approx 0.6$, an optimal policy is a simple threshold rule that observes the first $p^{1/(1-p)}$ fraction of candidates and subsequently makes offers to the best candidate observed so far.

==> Main3.tex <==
\section{Extension to multiple selection}

In many applications, multiple positions have to be fulfilled during the hiring season. Likewise, in many applications, companies can show the same ad multiple times. In this section, we extend the $\SPUA$ to a cardinality constraint. We utilize the MDP framework to derive the space of policies when a maximum amount of offers can be made and we utilize this to construct new policies (?)

The main results of this section are ... ta tan ..


\subsection{The space of policies}

The space of policies is given by
\[
\textsc{Pol}= \left\{ (x,y) : x_{1,1,\ell} + y_{1,1,\ell} = 1 , x_{t,s,\ell} + y_{t,s,\ell} = \frac{1}{t}\sum_{\sigma=1}^{t-1} y_{t-1,\sigma,\ell} + (1-p)x_{t-1,\sigma,\ell+1}, \forall t> 1,s,\ell  \right\}
\]





\subsection{Objective 1}




\subsection{Objective 2}
